4Real-Video: Learning Generalizable Photo-Realistic 4D Video Diffusion

We propose 4Real-Video, a novel framework for generating 4D videos, organized as a grid of video frames with both time and viewpoint axes. In this grid, each row contains frames sharing the same timestep, while each column contains frames from the same viewpoint. We propose a novel two-stream architecture. One stream performs viewpoint updates on columns, and the other stream performs temporal updates on rows. After each diffusion transformer layer, a synchronization layer exchanges information between the two token streams. We propose two implementations of the synchronization layer, using either hard or soft synchronization. This feedforward architecture improves upon previous work in three ways: higher inference speed, enhanced visual quality (measured by FVD, CLIP, and VideoScore), and improved temporal and viewpoint consistency (measured by VideoScore and Dust3R-Confidence).

==> figure_tex/videoscore_for_user_study.tex <==
\begin{table}[t!]
    \centering
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{c|c|ccccc}
    \toprule
         & X-CLIP $\uparrow$ & Visual Quality $\uparrow$ & Temporal Consistency$\uparrow$
         & Dynamic Degree
         $\uparrow$ & T-V Alignment $\uparrow$ & Factual Consistency $\uparrow$\\ 
    \midrule
    4Dfy~\cite{4dfy}  & 20.03 & 1.43 & 1.49 & 3.05 & 2.26 & 1.30 \\
    Ours & \textbf{24.23} & \textbf{2.43} & \textbf{2.17} & \textbf{3.15} & \textbf{2.91} & \textbf{2.49} \\
    \midrule
    Dream-in-4D~\cite{zheng2024unified} & 19.52 & 1.34 & 1.37 & 3.02 & 2.27 & 1.20 \\
    Ours & \textbf{24.77} & \textbf{2.41} & \textbf{2.15} & \textbf{3.14} & \textbf{2.89} & \textbf{2.46}\\
    \midrule
    AYG~\cite{aligngaussian} & 19.87 & \textbf{2.49} & 2.09 & 3.15 & 2.80 & 2.47 \\
    Ours & \textbf{23.09} & 2.44 & \textbf{2.16} & \textbf{3.16} & \textbf{2.90} & \textbf{2.50}\\
    \bottomrule
    \end{tabular}
    }
    \vspace{2mm}
    \caption{\textbf{Quantitative comparison against baselines} using X-CLIP~\cite{XCLIP} and VideoScore~\cite{videoscore}.}
    \vspace{-4mm}
    \label{tab:quan}
\end{table}


\begin{table}[t!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|cc|cc|cc|cc}
    \toprule
    Metric & Ours & 4Real~\cite{4real} & Ours & 4Dfy~\cite{4dfy} & Ours & Dream4D~\cite{zheng2024unified} & Ours & AYG~\cite{ayg}\\
    \midrule
    Visual Quality $\uparrow$ & 2.50 & 2.45 & &\\
    Temporal Consistency$\uparrow$ & 2.37 & 2.17\\
    Dynamic Degree $\uparrow$ & 3.03 & 3.16 \\
    T-V Alignment $\uparrow$ & 2.85 & 2.90\\
    Factual Consistency $\uparrow$ & 2.30 & 2.50 \
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Quantitative comparison against baselines using VideoScore~\cite{videoscore}.}}
    \label{tab:quan}
\end{table}

==> table_tex/quan_compare.tex <==
\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.1}
    \setlength{\tabcolsep}{2pt}  % default is 6pt, adjust as needed
    \begin{tabular}{ccccc}
        \toprule
    {Model} & {LPIPS} ($\downarrow$) & {CLIP} ($\uparrow$) &{FVD} ($\downarrow$) &{$\text{FD}_\text{DINO}$} ($\downarrow$) \\
        \hline
        SV4D~\cite{sv4d} &  0.0853 & 15.467 & 314.3428 &727.733\\
        % Ours &0.1323 &15.731 &420.4552  &760.758 \\

        \bottomrule
    \end{tabular}
    
    \caption{\textbf{Quantitative evaluation on 4D Objaverse dataset}~\cite{objaverse}.}
    \label{tab:compare}
\end{table}

